Incomplete decode-and-forward protocol using distributed space-time block codes

In this work, we explore the introduction of distributed space-time codes in decode-and-forward (DF) protocols. A first protocol named the Asymmetric DF is presented. It is based on two phases of different lengths, defined so that signals can be fully decoded at relays. This strategy brings full diversity but the symbol rate is not optimal. To solve this problem a second protocol named the Incomplete DF is defined. It is based on an incomplete decoding at the relays reducing the length of the first phase. This last strategy brings both full diversity and full symbol rate. The outage probability and the simulation results show that the Incomplete DF has better performance than any existing DF protocol and than the non-orthogonal amplify-and-forward (NAF) strategy using the same space-time codes. Moreover the diversity-multiplexing gain tradeoff (DMT) of this new DF protocol is proven to be the same as the one of the NAF.

==> figures/pout_1relai <==
<?xml version="1.0"?>
<grace version="59901" xmlns:grace="http://plasma-gate.weizmann.ac.il/Grace/">
 <!-- Description -->
 <description>
  <text/>
 </description>
 <!-- Definitions -->
 <definitions>
  <!-- Color map -->
  <colormap>
   <color-def id="0" rgb="#ffffff" name="white"/>
   <color-def id="1" rgb="#000000" name="black"/>
   <color-def id="2" rgb="#ff0000" name="red"/>
   <color-def id="3" rgb="#00ff00" name="green"/>
   <color-def id="4" rgb="#0000ff" name="blue"/>
   <color-def id="5" rgb="#ffff00" name="yellow"/>
   <color-def id="6" rgb="#bc8f8f" name="brown"/>
   <color-def id="7" rgb="#dcdcdc" name="grey"/>
   <color-def id="8" rgb="#9400d3" name="violet"/>
   <color-def id="9" rgb="#00ffff" name="cyan"/>
   <color-def id="10" rgb="#ff00ff" name="magenta"/>
   <color-def id="11" rgb="#ffa500" name="orange"/>
   <color-def id="12" rgb="#7221bc" name="indigo"/>
   <color-def id="13" rgb="#670748" name="maroon"/>
   <color-def id="14" rgb="#40e0d0" name="turquoise"/>
   <color-def id="15" rgb="#008b00" name="green4"/>
  </colormap>
  <!-- Font map -->
  <fontmap>
   <font-def id="0" name="Times-Roman" fallback="Times-Roman"/>
   <font-def id="1" name="Times-Italic" fallback="Times-Italic"/>
   <font-def id="2" name="Times-Bold" fallback="Times-Bold"/>
   <font-def id="3" name="Times-BoldItalic" fallback="Times-BoldItalic"/>
   <font-def id="4" name="Helvetica" fallback="Helvetica"/>
   <font-def id="5" name="Helvetica-Oblique" fallback="Helvetica-Oblique"/>
   <font-def id="6" name="Helvetica-Bold" fallback="Helvetica-Bold"/>
   <font-def id="7" name="Helvetica-BoldOblique" fallback="Helvetica-BoldOblique"/>
   <font-def id="8" name="Courier" fallback="Courier"/>
   <font-def id="9" name="Courier-Oblique" fallback="Courier-Oblique"/>
   <font-def id="10" name="Courier-Bold" fallback="Courier-Bold"/>
   <font-def id="11" name="Courier-BoldOblique" fallback="Courier-BoldOblique"/>
   <font-def id="12" name="Symbol" fallback="Symbol"/>
   <font-def id="13" name="ZapfDingbats" fallback="ZapfDingbats"/>
  </fontmap>
  <!-- Size scales -->
  <scales font-size="0.028" line-width="0.0015"/>
 </definitions>
 <!-- Page properties -->
 <page width="842" height="595" fill="yes" color-id="0"/>
 <!-- Data formats -->
 <data-formats>
  <world prec="8"/>
  <dates reference="0" wrap="no" wrap-year="1950"/>
 </data-formats>
 <frame id="frame" active="yes" type="closed">
  <viewport xmin="0.15" xmax="1.25" ymin="0.15" ymax="0.85"/>
  <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
  <fill-spec color-id="0" pattern-id="0"/>
  <legend active="yes" length="0.04" vgap="0.01" hgap="0.01" single-symbol="no" invert="no">
   <face-spec font-id="0" color-id="1" char-size="1"/>
   <legframe anchor="(1, 1)" offset="(-0.05, -0.05)" hjust="right" vjust="top">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="1"/>
   </legframe>
  </legend>
  <graph id="graph" active="yes">
   <presentation-spec type="xy" stacked="no" bargap="0"/>
   <xscale min="0" max="48" type="normal" invert="no"/>
   <yscale min="0.0001" max="1" type="logarithmic" invert="no"/>
   <zscale norm="1"/>
   <locator type="xy">
    <fixedpoint active="no" x="0" y="0"/>
    <xformat type="general" prec="6" format-string=""/>
    <yformat type="general" prec="6" format-string=""/>
   </locator>
   <agrid id="x_axisgrid" active="yes" type="x" major-step="10" minor-divisions="1" auto-ticking="6" rounded-position="yes">
    <major-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-gridlines>
    <minor-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-gridlines>
    <userticks type="none"/>
    <axisbar>
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </axisbar>
    <major-tickmarks size="1" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-tickmarks>
    <minor-tickmarks size="0.5" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-tickmarks>
    <ticklabels transform="" prepend="" append="" offset="(0, 0.01)" skip="0" stagger="0" start="auto" stop="auto">
     <text-properties angle="0" hjust="left" vjust="baseline">
      <face-spec font-id="0" color-id="1" char-size="1"/>
     </text-properties>
     <format type="general" prec="5" format-string=""/>
    </ticklabels>
    <axis id="normal" active="yes" position="normal" offset="0" bar="yes" ticks="yes" labels="yes">
     <atext id="label" active="yes" offset="(0, -0.01)">
      <location x="0.5" y="0"/>
      <text-properties angle="0" hjust="center" vjust="top">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <text><![CDATA[SNR (dB)]]></text>
      <text-frame type="none" offset="0.005">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
       <fill-spec color-id="0" pattern-id="0"/>
      </text-frame>
      <pointer active="no">
       <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
      </pointer>
     </atext>
    </axis>
    <axis id="opposite" active="yes" position="opposite" offset="0" bar="yes" ticks="yes" labels="no">
    </axis>
   </agrid>
   <agrid id="y_axisgrid" active="yes" type="y" major-step="10" minor-divisions="9" auto-ticking="6" rounded-position="yes">
    <major-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-gridlines>
    <minor-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-gridlines>
    <userticks type="none"/>
    <axisbar>
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </axisbar>
    <major-tickmarks size="1" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-tickmarks>
    <minor-tickmarks size="0.5" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-tickmarks>
    <ticklabels transform="" prepend="" append="" offset="(0, 0.01)" skip="0" stagger="0" start="auto" stop="auto">
     <text-properties angle="0" hjust="left" vjust="baseline">
      <face-spec font-id="0" color-id="1" char-size="1"/>
     </text-properties>
     <format type="power" prec="0" format-string=""/>
    </ticklabels>
    <axis id="normal" active="yes" position="normal" offset="0" bar="yes" ticks="yes" labels="yes">
     <atext id="label" active="yes" offset="(-0.01, 0)">
      <location x="0" y="0.5"/>
      <text-properties angle="90" hjust="right" vjust="middle">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <text><![CDATA[Outage probability]]></text>
      <text-frame type="none" offset="0.005">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
       <fill-spec color-id="0" pattern-id="0"/>
      </text-frame>
      <pointer active="no">
       <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
      </pointer>
     </atext>
    </axis>
    <axis id="opposite" active="yes" position="opposite" offset="0" bar="yes" ticks="yes" labels="no">
    </axis>
   </agrid>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_2bitspcu/SISO.data" active="yes" rows="16" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
     <c>39</c>
     <c>42</c>
     <c>45</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.792393</c>
     <c>0.52521</c>
     <c>0.318066</c>
     <c>0.169313</c>
     <c>0.089512</c>
     <c>0.046787</c>
     <c>0.023552</c>
     <c>0.011957</c>
     <c>0.005932</c>
     <c>0.002973</c>
     <c>0.001424</c>
     <c>0.000725</c>
     <c>0.000379</c>
     <c>0.000194</c>
     <c>1e-04</c>
     <c>4.6e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x83664b0" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="1" pattern-id="0" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="1" pattern-id="0" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[SISO - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_2bitspcu/NAF.data" active="yes" rows="10" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.896989</c>
     <c>0.659139</c>
     <c>0.411578</c>
     <c>0.193435</c>
     <c>0.066358</c>
     <c>0.018522</c>
     <c>0.004789</c>
     <c>0.001229</c>
     <c>0.000299</c>
     <c>7e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x873c258" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="2" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="2" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="3" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="2" pattern-id="0" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="2" pattern-id="0" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[NAF - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_2bitspcu/Partial DF.data" active="yes" rows="10" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.792393</c>
     <c>0.530987</c>
     <c>0.325382</c>
     <c>0.152672</c>
     <c>0.050888</c>
     <c>0.01532</c>
     <c>0.004385</c>
     <c>0.001163</c>
     <c>0.000293</c>
     <c>6.9e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
     <c>-0.124986</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x81ce388" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="triangle-up" size="0.5" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="1"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="3" pattern-id="0" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="3" pattern-id="0" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[Partial DF - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_4bitspcu/SISO.data" active="yes" rows="17" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
     <c>39</c>
     <c>42</c>
     <c>45</c>
     <c>48</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.972763</c>
     <c>0.84674</c>
     <c>0.604595</c>
     <c>0.384763</c>
     <c>0.209688</c>
     <c>0.115634</c>
     <c>0.055215</c>
     <c>0.029601</c>
     <c>0.014964</c>
     <c>0.007469</c>
     <c>0.003742</c>
     <c>0.001871</c>
     <c>0.000936</c>
     <c>0.000481</c>
     <c>0.000232</c>
     <c>0.000118</c>
     <c>5.8e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x8737cb8" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="4" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="4" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="4" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[SISO - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_4bitspcu/NAF.data" active="yes" rows="13" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
    </dcolumn>
    <dcolumn label="">
     <c>1</c>
     <c>0.936494</c>
     <c>0.775695</c>
     <c>0.529434</c>
     <c>0.307821</c>
     <c>0.165934</c>
     <c>0.070902</c>
     <c>0.025866</c>
     <c>0.006899</c>
     <c>0.001891</c>
     <c>0.00043</c>
     <c>0.000111</c>
     <c>2.6e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x8737b00" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="3" width="1"/>
      <fill-spec color-id="5" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="3" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="5" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="5" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[NAF - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim2/3relais/pout_4bitspcu/Partial DF.data" active="yes" rows="13" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.972763</c>
     <c>0.84674</c>
     <c>0.604595</c>
     <c>0.385533</c>
     <c>0.210736</c>
     <c>0.121994</c>
     <c>0.051943</c>
     <c>0.019866</c>
     <c>0.005605</c>
     <c>0.001674</c>
     <c>0.00041</c>
     <c>0.000108</c>
     <c>2.6e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x8742640" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="triangle-down" size="0.5" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="1"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="6" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="6" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[Partial DF - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <atext id="0x8778648" active="yes" offset="(0, 0)">
    <location x="5.8798133" y="0.015848215"/>
    <text-properties angle="0" hjust="left" vjust="baseline">
     <face-spec font-id="0" color-id="1" char-size="1"/>
    </text-properties>
    <text/>
    <text-frame type="none" offset="0.005">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
     <fill-spec color-id="0" pattern-id="0"/>
    </text-frame>
    <pointer active="no">
     <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
    </pointer>
   </atext>
  </graph>
  <atext id="title" active="no" offset="(0, 0.06)">
   <location x="0.5" y="1"/>
   <text-properties angle="0" hjust="left" vjust="baseline">
    <face-spec font-id="0" color-id="1" char-size="1.5"/>
   </text-properties>
   <text><![CDATA[Title]]></text>
   <text-frame type="none" offset="0.005">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="0"/>
   </text-frame>
   <pointer active="no">
    <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
   </pointer>
  </atext>
  <atext id="subtitle" active="no" offset="(0, 0.02)">
   <location x="0.5" y="1"/>
   <text-properties angle="0" hjust="left" vjust="baseline">
    <face-spec font-id="0" color-id="1" char-size="1"/>
   </text-properties>
   <text><![CDATA[Subtitle]]></text>
   <text-frame type="none" offset="0.005">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="0"/>
   </text-frame>
   <pointer active="no">
    <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
   </pointer>
  </atext>
 </frame>
 <atext id="timestamp" active="no" offset="(0, 0)">
  <location x="0.03" y="0.03"/>
  <text-properties angle="0" hjust="left" vjust="baseline">
   <face-spec font-id="0" color-id="1" char-size="1"/>
  </text-properties>
  <text><![CDATA[\${timestamp}]]></text>
  <text-frame type="none" offset="0">
   <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
   <fill-spec color-id="0" pattern-id="0"/>
  </text-frame>
  <pointer active="no">
   <arrow type="line" length="0" dl-ff="0" ll-ff="0"/>
  </pointer>
 </atext>
</grace>


==> figures/pout_2relais <==
<?xml version="1.0"?>
<grace version="59901" xmlns:grace="http://plasma-gate.weizmann.ac.il/Grace/">
 <!-- Description -->
 <description>
  <text/>
 </description>
 <!-- Definitions -->
 <definitions>
  <!-- Color map -->
  <colormap>
   <color-def id="0" rgb="#ffffff" name="white"/>
   <color-def id="1" rgb="#000000" name="black"/>
   <color-def id="2" rgb="#ff0000" name="red"/>
   <color-def id="3" rgb="#00ff00" name="green"/>
   <color-def id="4" rgb="#0000ff" name="blue"/>
   <color-def id="5" rgb="#ffff00" name="yellow"/>
   <color-def id="6" rgb="#bc8f8f" name="brown"/>
   <color-def id="7" rgb="#dcdcdc" name="grey"/>
   <color-def id="8" rgb="#9400d3" name="violet"/>
   <color-def id="9" rgb="#00ffff" name="cyan"/>
   <color-def id="10" rgb="#ff00ff" name="magenta"/>
   <color-def id="11" rgb="#ffa500" name="orange"/>
   <color-def id="12" rgb="#7221bc" name="indigo"/>
   <color-def id="13" rgb="#670748" name="maroon"/>
   <color-def id="14" rgb="#40e0d0" name="turquoise"/>
   <color-def id="15" rgb="#008b00" name="green4"/>
  </colormap>
  <!-- Font map -->
  <fontmap>
   <font-def id="0" name="Times-Roman" fallback="Times-Roman"/>
   <font-def id="1" name="Times-Italic" fallback="Times-Italic"/>
   <font-def id="2" name="Times-Bold" fallback="Times-Bold"/>
   <font-def id="3" name="Times-BoldItalic" fallback="Times-BoldItalic"/>
   <font-def id="4" name="Helvetica" fallback="Helvetica"/>
   <font-def id="5" name="Helvetica-Oblique" fallback="Helvetica-Oblique"/>
   <font-def id="6" name="Helvetica-Bold" fallback="Helvetica-Bold"/>
   <font-def id="7" name="Helvetica-BoldOblique" fallback="Helvetica-BoldOblique"/>
   <font-def id="8" name="Courier" fallback="Courier"/>
   <font-def id="9" name="Courier-Oblique" fallback="Courier-Oblique"/>
   <font-def id="10" name="Courier-Bold" fallback="Courier-Bold"/>
   <font-def id="11" name="Courier-BoldOblique" fallback="Courier-BoldOblique"/>
   <font-def id="12" name="Symbol" fallback="Symbol"/>
   <font-def id="13" name="ZapfDingbats" fallback="ZapfDingbats"/>
  </fontmap>
  <!-- Size scales -->
  <scales font-size="0.028" line-width="0.0015"/>
 </definitions>
 <!-- Page properties -->
 <page width="842" height="595" fill="yes" color-id="0"/>
 <!-- Data formats -->
 <data-formats>
  <world prec="8"/>
  <dates reference="0" wrap="no" wrap-year="1950"/>
 </data-formats>
 <frame id="frame" active="yes" type="closed">
  <viewport xmin="0.15" xmax="1.25" ymin="0.15" ymax="0.85"/>
  <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
  <fill-spec color-id="0" pattern-id="0"/>
  <legend active="yes" length="0.04" vgap="0.01" hgap="0.01" single-symbol="no" invert="no">
   <face-spec font-id="0" color-id="1" char-size="1"/>
   <legframe anchor="(1, 1)" offset="(-0.05, -0.05)" hjust="right" vjust="top">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="1"/>
   </legframe>
  </legend>
  <graph id="graph" active="yes">
   <presentation-spec type="xy" stacked="no" bargap="0"/>
   <xscale min="0" max="48" type="normal" invert="no"/>
   <yscale min="0.0001" max="1" type="logarithmic" invert="no"/>
   <zscale norm="1"/>
   <locator type="xy">
    <fixedpoint active="no" x="0" y="0"/>
    <xformat type="general" prec="6" format-string=""/>
    <yformat type="general" prec="6" format-string=""/>
   </locator>
   <agrid id="x_axisgrid" active="yes" type="x" major-step="10" minor-divisions="1" auto-ticking="6" rounded-position="yes">
    <major-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-gridlines>
    <minor-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-gridlines>
    <userticks type="none"/>
    <axisbar>
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </axisbar>
    <major-tickmarks size="1" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-tickmarks>
    <minor-tickmarks size="0.5" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-tickmarks>
    <ticklabels transform="" prepend="" append="" offset="(0, 0.01)" skip="0" stagger="0" start="auto" stop="auto">
     <text-properties angle="0" hjust="left" vjust="baseline">
      <face-spec font-id="0" color-id="1" char-size="1"/>
     </text-properties>
     <format type="general" prec="5" format-string=""/>
    </ticklabels>
    <axis id="normal" active="yes" position="normal" offset="0" bar="yes" ticks="yes" labels="yes">
     <atext id="label" active="yes" offset="(0, -0.01)">
      <location x="0.5" y="0"/>
      <text-properties angle="0" hjust="center" vjust="top">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <text><![CDATA[SNR (dB)]]></text>
      <text-frame type="none" offset="0.005">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
       <fill-spec color-id="0" pattern-id="0"/>
      </text-frame>
      <pointer active="no">
       <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
      </pointer>
     </atext>
    </axis>
    <axis id="opposite" active="yes" position="opposite" offset="0" bar="yes" ticks="yes" labels="no">
    </axis>
   </agrid>
   <agrid id="y_axisgrid" active="yes" type="y" major-step="10" minor-divisions="9" auto-ticking="6" rounded-position="yes">
    <major-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-gridlines>
    <minor-gridlines active="no">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-gridlines>
    <userticks type="none"/>
    <axisbar>
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </axisbar>
    <major-tickmarks size="1" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </major-tickmarks>
    <minor-tickmarks size="0.5" inout-placement="in">
     <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    </minor-tickmarks>
    <ticklabels transform="" prepend="" append="" offset="(0, 0.01)" skip="0" stagger="0" start="auto" stop="auto">
     <text-properties angle="0" hjust="left" vjust="baseline">
      <face-spec font-id="0" color-id="1" char-size="1"/>
     </text-properties>
     <format type="power" prec="0" format-string=""/>
    </ticklabels>
    <axis id="normal" active="yes" position="normal" offset="0" bar="yes" ticks="yes" labels="yes">
     <atext id="label" active="yes" offset="(-0.01, 0)">
      <location x="0" y="0.5"/>
      <text-properties angle="90" hjust="right" vjust="middle">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <text><![CDATA[Outage probability]]></text>
      <text-frame type="none" offset="0.005">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
       <fill-spec color-id="0" pattern-id="0"/>
      </text-frame>
      <pointer active="no">
       <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
      </pointer>
     </atext>
    </axis>
    <axis id="opposite" active="yes" position="opposite" offset="0" bar="yes" ticks="yes" labels="no">
    </axis>
   </agrid>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/2bitspcu/SISO.data" active="yes" rows="15" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
     <c>39</c>
     <c>42</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.792393</c>
     <c>0.52521</c>
     <c>0.316317</c>
     <c>0.171081</c>
     <c>0.090215</c>
     <c>0.046412</c>
     <c>0.023613</c>
     <c>0.011823</c>
     <c>0.005947</c>
     <c>0.002997</c>
     <c>0.001471</c>
     <c>0.000763</c>
     <c>0.000392</c>
     <c>0.00018</c>
     <c>9.1e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x8743620" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[SISO - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/2bitspcu/NAF.data" active="yes" rows="9" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.887924</c>
     <c>0.67112</c>
     <c>0.423077</c>
     <c>0.211763</c>
     <c>0.076843</c>
     <c>0.018136</c>
     <c>0.002871</c>
     <c>0.000395</c>
     <c>5.1e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x87314b0" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="2" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="2" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="3" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="2" pattern-id="0" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="2" pattern-id="0" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[NAF - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/2bitspcu/Partial_DF.data" active="yes" rows="9" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.789266</c>
     <c>0.514902</c>
     <c>0.326761</c>
     <c>0.162022</c>
     <c>0.054654</c>
     <c>0.012355</c>
     <c>0.00212</c>
     <c>0.000349</c>
     <c>4.9e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
     <c>-0.78893</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x87d7800" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="triangle-up" size="0.5" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="1"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="3" pattern-id="0" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="3" pattern-id="0" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[Partial DF - 2 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/4bitspcu/SISO.data" active="yes" rows="17" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
     <c>36</c>
     <c>39</c>
     <c>42</c>
     <c>45</c>
     <c>48</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.972763</c>
     <c>0.84317</c>
     <c>0.611995</c>
     <c>0.379795</c>
     <c>0.210615</c>
     <c>0.112271</c>
     <c>0.055175</c>
     <c>0.029129</c>
     <c>0.014758</c>
     <c>0.007395</c>
     <c>0.003759</c>
     <c>0.001875</c>
     <c>0.000955</c>
     <c>0.00048</c>
     <c>0.000244</c>
     <c>0.000118</c>
     <c>5.8e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x81fae60" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="4" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="4" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="4" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="4" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[SISO - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/4bitspcu/NAF.data" active="yes" rows="12" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.998054</c>
     <c>0.94688</c>
     <c>0.78519</c>
     <c>0.529054</c>
     <c>0.315501</c>
     <c>0.167621</c>
     <c>0.075866</c>
     <c>0.029495</c>
     <c>0.007452</c>
     <c>0.001229</c>
     <c>0.000188</c>
     <c>2.6e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x873ef18" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="none" size="1" char="65" font-id="0">
      <line-spec color-id="5" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="5" pattern-id="0"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="3" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="5" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="5" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[NAF - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
   <ssd id="/comelec/these/hucher/Desktop/data/relay_channel/dim4/pout/4relais/new_DF/4bitspcu/Partial_DF.data" active="yes" rows="12" indexed="no">
    <dcolumn label="">
     <c>0</c>
     <c>3</c>
     <c>6</c>
     <c>9</c>
     <c>12</c>
     <c>15</c>
     <c>18</c>
     <c>21</c>
     <c>24</c>
     <c>27</c>
     <c>30</c>
     <c>33</c>
    </dcolumn>
    <dcolumn label="">
     <c>0.972763</c>
     <c>0.84317</c>
     <c>0.611995</c>
     <c>0.379795</c>
     <c>0.210826</c>
     <c>0.115864</c>
     <c>0.055562</c>
     <c>0.020313</c>
     <c>0.00507</c>
     <c>0.000922</c>
     <c>0.000156</c>
     <c>2.3e-05</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <dcolumn label="">
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
     <c>0</c>
    </dcolumn>
    <set id="0x8785b00" active="yes" type="xy" skip="0" skipmindist="0">
     <dataset x="0" y="1" y1="2" y2="3"/>
     <symbol type="triangle-down" size="0.5" char="65" font-id="0">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="1" pattern-id="1"/>
     </symbol>
     <line type="straight" fill-type="none" fill-rule="winding" baseline-type="zero" draw-baseline="no" draw-droplines="no">
      <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
      <fill-spec color-id="0" pattern-id="0"/>
     </line>
     <annotation active="no" offset="(0, 0)" prepend="" append="">
      <text-properties angle="0" hjust="center" vjust="bottom">
       <face-spec font-id="0" color-id="1" char-size="1"/>
      </text-properties>
      <format type="general" prec="3" format-string=""/>
     </annotation>
     <errorbar active="yes">
      <barline size="1">
       <line-spec color-id="6" pattern-id="1" style-id="1" width="1"/>
      </barline>
      <riserline arrow-clip="no" clip-length="0.1">
       <line-spec color-id="6" pattern-id="1" style-id="1" width="1"/>
      </riserline>
     </errorbar>
     <legend-entry>
      <text><![CDATA[Partial DF - 4 bits pcu]]></text>
     </legend-entry>
    </set>
   </ssd>
  </graph>
  <atext id="title" active="no" offset="(0, 0.06)">
   <location x="0.5" y="1"/>
   <text-properties angle="0" hjust="left" vjust="baseline">
    <face-spec font-id="0" color-id="1" char-size="1.5"/>
   </text-properties>
   <text><![CDATA[Title]]></text>
   <text-frame type="none" offset="0.005">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="0"/>
   </text-frame>
   <pointer active="no">
    <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
   </pointer>
  </atext>
  <atext id="subtitle" active="no" offset="(0, 0.02)">
   <location x="0.5" y="1"/>
   <text-properties angle="0" hjust="left" vjust="baseline">
    <face-spec font-id="0" color-id="1" char-size="1"/>
   </text-properties>
   <text><![CDATA[Subtitle]]></text>
   <text-frame type="none" offset="0.005">
    <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
    <fill-spec color-id="0" pattern-id="0"/>
   </text-frame>
   <pointer active="no">
    <arrow type="line" length="1" dl-ff="1" ll-ff="0"/>
   </pointer>
  </atext>
 </frame>
 <atext id="timestamp" active="no" offset="(0, 0)">
  <location x="0.03" y="0.03"/>
  <text-properties angle="0" hjust="left" vjust="baseline">
   <face-spec font-id="0" color-id="1" char-size="1"/>
  </text-properties>
  <text><![CDATA[\${timestamp}]]></text>
  <text-frame type="none" offset="0">
   <line-spec color-id="1" pattern-id="1" style-id="1" width="1"/>
   <fill-spec color-id="0" pattern-id="0"/>
  </text-frame>
  <pointer active="no">
   <arrow type="line" length="0" dl-ff="0" ll-ff="0"/>
  </pointer>
 </atext>
</grace>

